MDTD: A Multi Domain Trojan Detector for Deep Neural Networks

Machine learning models that use deep neural networks (DNNs) are vulnerable to backdoor attacks. An adversary carrying out a backdoor attack embeds a predefined perturbation called a trigger into a small subset of input samples and trains the DNN such that the presence of the trigger in the input results in an adversary-desired output class. Such adversarial retraining however needs to ensure that outputs for inputs without the trigger remain unaffected and provide high classification accuracy on clean samples. In this paper, we propose MDTD, a Multi-Domain Trojan Detector for DNNs, which detects inputs containing a Trojan trigger at testing time. MDTD does not require knowledge of trigger-embedding strategy of the attacker and can be applied to a pre-trained DNN model with image, audio, or graph-based inputs. MDTD leverages an insight that input samples containing a Trojan trigger are located relatively farther away from a decision boundary than clean samples. MDTD estimates the distance to a decision boundary using adversarial learning methods and uses this distance to infer whether a test-time input sample is Trojaned or not. We evaluate MDTD against state-of-the-art Trojan detection methods across five widely used image-based datasets: CIFAR100, CIFAR10, GTSRB, SVHN, and Flowers102; four graph-based datasets: AIDS, WinMal, Toxicant, and COLLAB; and the SpeechCommand audio dataset. MDTD effectively identifies samples that contain different types of Trojan triggers. We evaluate MDTD against adaptive attacks where an adversary trains a robust DNN to increase (decrease) distance of benign (Trojan) inputs from a decision boundary.

==> background.tex <==
\section{Background and Related Work}
\label{sec:relwork}
In~\secref{sec:intro} you talked about the project at a very high-level. This is
the section from where you will start giving details. First with things that are
already done, and familiarize the reader with background information they will
need to understand you work. 


\paragraph{Threat model.}
Often this section you will discuss the threat-model, but there is no strict consensus on that. 


Here is how you cite papers. For example, we read papers in the
class~\cite{rahul2016pwtypos,dodisetal:2004}.  And here is some random citation~\cite{Bojinov:2010:KLP,schechter:2010:pen,everspaugh2015pythia,bellare2009format,Juels:2014}


\subsection{Overview of the design}
\label{sec:overview}

And then just to showoff some \LaTeX skills, here is a Tikz plot.
\input{images/mainflow.tex}

You refer to a figure in the following way. In~\figref{fig:mainflow} we show
some thing that is relevant for the Multisketch paper by Chatterjee et
al.~\cite{chatterjee2019multisketches}. Add your bibliography to the
\textsf{bib.bib} file. You can copy the Bibtex format citation from Google
Scholar.

